On the Design of Communication and Transaction Anonymity in Blockchain-Based Transactive Microgrids

Transactive microgrids are emerging as a transformative solution for the problems faced by distribution system operators due to an increase in the use of distributed energy resources and a rapid acceleration in renewable energy generation, such as wind and solar power. Distributed ledgers have recently found widespread interest in this domain due to their ability to provide transactional integrity across decentralized computing nodes. However, the existing state of the art has not focused on the privacy preservation requirement of these energy systems -- the transaction level data can provide much greater insights into a prosumer's behavior compared to smart meter data. There are specific safety requirements in transactive microgrids to ensure the stability of the grid and to control the load. To fulfil these requirements, the distribution system operator needs transaction information from the grid, which poses a further challenge to the privacy-goals. This problem is made worse by requirement for off-blockchain communication in these networks. In this paper, we extend a recently developed trading workflow called PETra and describe our solution for communication and transactional anonymity.

==> figArchitecture.tex <==
\begin{figure*}
\center
\begin{tikzpicture}[
  x=1cm, 
  y=1cm,
  nodeStyle/.style={fill=white, draw=black, drop shadow=black!30, minimum size=0.5cm},
  linkStyle/.style={<->, >=stealth, shorten >=1.5pt, shorten <=1.5pt},
  batchStyle/.style={->, very thick, >=stealth},
  braceStyle/.style={decorate, decoration={brace,amplitude=0.2cm}, yshift=-0.4cm},
]

% trading nodes
\begin{scope}[xshift=1cm]

\foreach \name/\x/\y in {{t1/0/0}, {t2/1/1.4}, {t3/2/0}}
  \node [nodeStyle, regular polygon, regular polygon sides=5] (\name) at (\x,\y) {};

\foreach \name/\x/\y in {{tRight/2.5/0.7}}
  \coordinate (\name) at (\x,\y);

\foreach \from/\to in {{t1/t2}, {t2/t3}, {t3/t1}}
  \draw [linkStyle] (\from) -- (\to);
  
\draw [braceStyle] (2.25, 0) -- (-0.25, 0) node [midway, below=0.2cm] {trading nodes};
\end{scope}

% prosumer nodes
\begin{scope}[xshift=6cm]

\foreach \name/\x/\y in {{p1/0/0}, {p2/1.4/0}, {p3/0/1.4}, {p4/1.4/1.4}}
  \node [nodeStyle, rounded corners=0.1cm] (\name) at (\x,\y) {};

\foreach \name/\x/\y in {{pLeft/-0.6/0.7}, {pRight/2/0.7}}
  \coordinate (\name) at (\x,\y);

\foreach \from/\to in {{p1/p2}, {p1/p3}, {p1/p4}, {p2/p3}, {p2/p4}, {p3/p4}}
  \draw [linkStyle, dashed] (\from) -- (\to);
  
\draw [braceStyle] (1.65, 0) -- (-0.25, 0) node [midway, below=0.2cm] {prosumer nodes};
\end{scope}

% smart-meter nodes
\begin{scope}[xshift=6cm, yshift=2.7cm]

\foreach \name/\x/\y in {{m1/0/0}, {m2/1.4/0}, {m3/0/1.4}, {m4/1.4/1.4}}
  \node [diamond, nodeStyle] (\name) at (\x,\y) {};

\foreach \name/\x/\y in {{mRight/2/0.7}}
  \coordinate (\name) at (\x,\y);

\foreach \from/\to in {{m1/m2}, {m1/m3}, {m1/m4}, {m2/m3}, {m2/m4}, {m3/m4}}
  \draw [linkStyle, dashed] (\from) -- (\to);
  
\draw [braceStyle, yshift=0.8cm] (-0.25, 1.4) -- (1.65, 1.4) node [midway, above=0.2cm] {smart-meter nodes};
\end{scope}

% ledger nodes
\begin{scope}[xshift=11.5cm]

\foreach \name/\x/\y in {{l1/0/0}, {l2/1/1.4}, {l3/2/0}}
  \node [circle, nodeStyle] (\name) at (\x,\y) {};

\foreach \name/\x/\y in {{lLeft/-0.5/0.7}, {lTopLeft/0/1.6}, {lTopRight/1.6/1.0}}
  \coordinate (\name) at (\x,\y);

\foreach \from/\to in {{l1/l2}, {l2/l3}, {l3/l1}}
  \draw [<->, >=stealth, shorten >=1.5pt, shorten <=1.5pt] (\from) -- (\to);
  
\draw [decorate, decoration={brace,amplitude=0.2cm}, yshift=-0.4cm] (2.25, 0) -- (-0.25, 0) node [midway, below=0.2cm] {ledger nodes};
\end{scope}

% additional nodes
\node [ellipse, nodeStyle] (dso) at (15cm, 3.1cm) {DSO node};

\draw [->, >=stealth, bend right=10, shorten <=0.25cm, shorten >=0.5cm] (dso) to node [midway, above left=0cm, align=center] {regulatory\\[-0.25em]transactions} (lTopRight);
\draw [<-, >=stealth, bend left=10, shorten <=0.25cm, shorten >=0.5cm] (dso) to node [midway, below right=0cm, align=center] {ledger status} (lTopRight);

\node [above=1.2cm of dso] (controller) {control algorithm}; 

\draw [<-, >=stealth, bend right=10, shorten <=1.5pt] (dso) to node [midway, left=0.3cm, align=center] {measured and\\[-0.25em]expected load} (controller);
\draw [->, >=stealth, bend left=10, shorten <=1.5pt] (dso) to node [midway, right=0.3cm, align=center] {control\\[-0.25em]signal} (controller);

% connections between systems
\draw [batchStyle, <-, bend left=5] (tRight) to node [midway, above=0.1cm] {bids} (pLeft);
\draw [batchStyle, bend right=5] ([yshift=-0.4cm]tRight) to node [midway, below=0.1cm] {matches} ([yshift=-0.4cm]pLeft);

\draw [batchStyle, bend left=5] (pRight) to node [midway, above=0.1cm, align=center] {financial\\[-0.25em]transactions} ([yshift=0cm]lLeft);
\draw [batchStyle, <-, bend right=5] ([yshift=-0.4cm]pRight) to node [midway, below=0.1cm] {ledger status} ([yshift=-0.4cm]lLeft);

\draw [batchStyle, bend left=15] ([yshift=0.2cm]mRight) to node [midway, above right=0cm, align=center] {energy\\[-0.25em]transactions} ([yshift=0.2cm]lTopLeft);
\draw [batchStyle, <-, bend right=-5] ([yshift=-0.2cm]mRight) to node [midway, below left=0cm] {ledger status} ([yshift=-0.2cm]lTopLeft);

\end{tikzpicture}
\caption{High-level logical architecture of the trading platform and the distributed ledger. A physical node may implement multiple logical nodes.}
\label{fig:logicalNodeArchitecture}
\end{figure*}


